Strange Duality for elliptic surfaces

The main result of the present paper is the proof of the Strange Duality for elliptic surfaces -- a duality between global sections of determinantal line bundles on moduli spaces of stable sheaves on a fixed elliptic surface. For this, we employ the "Marian-Oprea trick": using Bridgeland's birational isomorphisms, we reduce the problem from a pair of general moduli spaces to a pair of Hilbert schemes. The latter case is a theorem by Marian-Oprea.

==> body/13.tex <==
%%%
\subsection{Computing Chern characters}
\label{Subsec:matrices:Chern}
%%%



\begin{Prop}
    On $X\times X$:
$$
\ch \iota_* \Oc_\Pi(-\Delta)=
\Pi
-\left([f\times f]+\Delta \right)
+ 2[*] 
.$$
\end{Prop}


\begin{Lem}
$$
\ch \Oc_{X\times X} ((d+1)[\sigma\times X]) =
1 + (d+1)[\sigma\times X]
- (d+1)^2 [*\times X]
.$$
\end{Lem}

\begin{Lem}
$$
\ch \Oc_{X\times X} ([X\times\sigma]) =
1 + [X\times\sigma] 
- [X\times *]
.$$
\end{Lem}

\begin{Lem}
\begin{equation*}
\begin{split}
\ch \rho^* \Oc_{\PS^1} (2(d+1)) &=
\iota^*(1+2(d+1)[f\times X])\\
&=\iota^*(1+2(d+1)[X\times f])
\end{split}
\end{equation*} 
\end{Lem}

==> body/SDmodern.tex <==
\section{Modern view on the Strange Duality}

Strange Duality = projective duality of projective bundles

Theta locus = locus where RHom is less trivial

Orthogonality is used in the construction of Verlinde sheaves

K3 surfaces: no difference between $\Kt$ and $\Kor$

Curves: no difference between $\K$ and $\Kor$

Why do we get different K-theories?

==> body/building_expl_kernels.tex <==
\section{Building up Strange Duality}
\label{building_expl}


%%%
%%%
\subsection{Zooming in: two explicit kernels}
%%%
%%%


Let $X$ be an elliptic K3 surface with $\pi : X \to \PS^1$ being the elliptic fibration. Let $H$ be a quasipolarization on $X$.
Let $\Pi \deq X \times_{\PS^1} X$ -- it is a divisor in $X \times X$, and let $\iota : \Pi \to X \times X$ denote the embedding.
Let $\Delta \cong X$ be the diagonal, and let $\delta : \Delta \to X \times X$ denote the diagonal embedding.
Let $p$ and $q$ denote two projections from $X \times X$ to $X$. These notation can be summarized in the following diagram:
\begin{diagram}
\Delta \cong X  & \rInto            & \Pi           & \Ic_\Delta    \\
                & \rdInto_\delta    & \dInto_\iota                  \\
                &                   & X \times X    & \Ic           \\
                & \ldTo^p           &               & \rdTo^q       \\
X               &                   &               &           & X
\end{diagram}

In this case, we want to study two types of explicit kernels defining autoequivalences of $\Db X$:
\begin{itemize}
    \item
    First we have
    $\Ic \deq \iota_* \Ic_\Delta$
    -- the pushforward from $\Pi$ of the ideal sheaf of the diagonal
    $\Delta \subset \Pi$.
    We will denote the corresponding Fourier-Mukai functor by
    $$ S \deq q_*(\Ic \otimes p^*(-)). $$
    \item
    Next, we have the kernel corresponding to a twist by a line bundle
    $L \in \Pic X$ is
    $\Oc_\Delta \otimes q^* L$.
    The corresponding Fourier-Mukai equivalence will be denoted by
    $$ T_L \deq q_*(\Oc_\Delta \otimes q^*L \otimes p^*(-)). $$
\end{itemize}

We want to use a composition of these kernels to generalize Strange Duality from the Marian-Oprea case \cite{MO}:
\begin{equation*}
    v = (r_v, H, k_v) \mbox{, } 
    w = (r_w, H, k_w) \mbox{, } 
    H^2 > 2
\end{equation*}
to the case with more general $\cn_1(v)$ and $\cn_1(w)$ and no assumption on the degree $H^2$ of $X$:
\begin{equation*}
    v = (r_v, \Lambda_v, k_v) \mbox{, }
    w = (r_w, \Lambda_w, k_w) \mbox{.}
\end{equation*}

We will start with explaining how kernels of types S and T act on the Chern classes and then apply this knowledge to produce more general Strange Duality isomorphisms.



%%%
\subsubsection{Chern character of $\Ic$}
%%%



\begin{Lem}
    The Todd class of $X \times X$ is equal to the following expression:
    $$ \td\!_{X\times X} = 1 +
    2([X\times*] + [*\times X]) + 4[*]
    \mbox{.} $$
\end{Lem}

\begin{proof}
Use that the tangent bundle on $X \times X$ is isomorphic to $p^* \Tc_X \oplus q^* \Tc_X$ and multiplicativity of Todd class.
\end{proof}

\begin{Lem}
    The Chern character of $\Ic = \iota_* \Ic_\Delta$ is equal to the following expression:
    $$ \ch \Ic = \Pi -
        \left(\frac{\Pi^2}{2} + \Delta\right)
        + \frac{\Pi^3}{6} +
        \left( 2[*] - \frac{\Pi^4}{24} \right)
    \mbox{.} $$
\end{Lem}

\begin{proof}
We have the following short exact sequence on $\Pi$:
$$  0 \to \Ic_\Delta \to \Oc_\Pi \to \Oc_\Delta \to 0 \mbox{.} $$
Since $\iota$ is a closed embedding, the functor $\iota_*$ is exact, so we also have a short exact sequence on $X \times X$:
$$  0 \to \Ic \to \Oc_\Pi \to \Oc_\Delta \to 0 \mbox{.} $$
Then $\ch \Ic = \ch \Oc_\Pi - \ch \Oc_\Delta$. Note that since $\Pi$ is a divisor, we have a short exact sequence on $X \times X$:
$$  0 \to \Oc(-\Pi) \to \Oc \to \Oc_\Pi \to 0
\mbox{,} $$
and moreover,
$\ch \Oc(-\Pi) = 1-\Pi+\frac{\Pi^2}{2}-
\frac{\Pi^3}{6}+\frac{\Pi^4}{24}$.

Next, by Grothendieck-Riemann-Roch and noting that $\delta_! = \delta_*$, we get
$(\ch \delta_* \Oc_\Delta).\td\!_{X\times X} = \delta_* ((\ch \Oc_\Delta).\td\!_\Delta) =
\delta_* (1 + 2[*]) = \Delta + 2[*]$.

Now we need to invert the Todd class $\td\!_{X\times X}$ to compute the Chern class. But note that $\Delta + 2[*]$ has lowest degree two, therefore we can forget about the degree four part of the Todd class. Then
$\ch \Oc_\Delta = (\Delta + 2[*]).(1-
2([X\times*] + [*\times X])) =
\Delta + 2[*] -2\cdot2 [*] = \Delta - 2[*]$.

Finally, we can plug in the acquired formulas to get the desired
$\ch \Ic = \ch \Oc_\Pi - \ch \Oc_\Delta =
\ch \Oc - \ch \Oc(-\Pi) - \ch \Oc_\Delta$.
\end{proof}



%%%
\subsubsection{Action of $S$ on Chern classes}
%%%


\begin{Lem}
    For an object $E \in \Db X$, we have:
    \begin{itemize}
        \item $\rk SE = - \rk E + \fdeg E$;
        \item $\det SE = \det E^\vee \otimes \Fc$, where $\Fc \cong \Oc_X \left( \left( 2r - \fdeg E + \chn_2 E \right)f \right)$ is a line bundle corresponding to a multiple of the fiber class;
        \item $\chn_2 SE = -\chn_2 E$.
    \end{itemize}
\end{Lem}

\begin{proof}
We can rewrite the class of $SE$ in $\K X$ as follows:
\begin{equation*}
\begin{split}
    [SE] &= 
    \left[ q_*(\Ic \otimes p^* E) \right]=
    q_* \left( 
    \left( \left[ \Oc_\Pi \right] - \left[ \Oc_\Delta \right] \right)
    \otimes \left[ p^*E \right] \right) =\\
    &= \left[ q_*(\Oc_\Pi \otimes p^*E)
        \right] -
        \left[ q_*(\Oc_\Delta \otimes p^*E) \right]
\mbox{.} \end{split}
\end{equation*}

Now denote by $\bar p$ and $\bar q$ the two projections from the fiber product $\Pi$ to $X$. Then by projection formula, we get
$   \left[ q_*(\Oc_\Pi \otimes p^*E)
        \right] =
    \left[ \bar q_* \bar p^*E \right]$.
Further, Fourier-Mukai functor whose kernel is the structure sheaf of the diagonal is naturally isomorphic to the identity functor, hence
$\left[ q_*(\Oc_\Delta \otimes p^*E) \right]
= [E]$.
As a consequence, we can further simplify our expression for $[SE]$:
$$  [SE] =
    \left[ \bar q_* \bar p^*E \right]
    -   [E]
. $$
Then, by base change, this is equal to:
$$  [SE] = \left[ \pi^*\pi_* E \right] - [E]
\mbox{.} $$

Since the Chern character is a ring homomorphism from the Grothendieck group, we get that $\ch SE = - \ch E + \ch (\pi^* \pi_* E) =
- \ch E + \pi^* \ch \pi_* E$. To get the desired formulas, it is enough to calculate $\ch \pi_* E$, and automatically $\chn_2 SE = -\chn_2 E$, because $\PS^1$ is one-dimensional and therefore $\pi^* \ch \pi_* E$ is of degree at most one.

Let's put $\ch E = r + E_1 + E_2[*]$ and apply Grothendieck-Riemann-Roch:
\begin{equation*}
\begin{split}
    (\ch \pi_* E).\td_{\PS^1} &=
        \pi_* (\ch E . \td_X) =
        \pi_* ((r+E_1+E_2[*]).(1+2[*])) =\\
    &= \pi_* (r+E_1+(E_2 + 2r)[*]) =
        \pi_* E_1 + (E_2+2r)[*] \mbox{;}\\
    \ch \pi_* E &=
        (\ch \pi_* E).\td_{\PS^1}.
        \td_{\PS^1}^{-1} =
        (\pi_*E_1+(E_2+2r)[*]).(1-[*]) =\\
    &= \pi_*E_1 + (E_2+2r-\pi_*E_1)[*]
    \mbox{.} \\
\end{split}
\end{equation*}

From this formula we observe that $\pi_*E_1 = \rk \pi_*E = \fdeg E$, therefore:
\begin{equation*}
\begin{split}
    \det \pi_* E &= \cn_1 \pi_* E =
    E_2+2r-\pi_*E_1 =
    2r - \fdeg E + E_2
\mbox{;}\\
    \rk \pi^* \pi_* E &= \rk \pi_* E = \fdeg E
\mbox{.}
\end{split}
\end{equation*}

From this, we are able to immediately deduce the formulas.
\end{proof}

For convenience, we will write the action of $S$ on the Chow groups as a $3 \times 3$ matrix. 

\begin{Not}
    Let us introduce notation for the matrices:
    \begin{itemize}
    \item three-by-three matrix that represents the action of a functor $F: \Db X$ $\to \Db X$ on the vector of rank, first Chern class and second graded component of Chern character will be denoted by $A_F$, and the Chern character is viewed as an element of either topological or oriented topological K-group;
    \item two-by-two Bridgeland matrix that represents the action of $F$ on the vector of rank and fiber degree will be denoted by $B_F$.
    \end{itemize}
\end{Not}

\paragraph{Convention.}
Since entries of the matrix are not just multiplications by an element of the ring $\Chow X$, we will view them as elements of the (noncommutative graded) ring of endomorphisms of $\Chow X$. Intersection product with a cycle $\alpha$ will be denoted by $\hat\alpha$, the homomorphism of taking degree of a two-cycle will be denoted by $\deg$ and is of degree $-2$, and the homomorphism of taking fiber degree will be denoted by $\fdeg$ and has degree $-1$. The symbol $\circ$ will denote composition of endomorphisms, as is customary. In addition, when writing $\ch E$, we will sometimes mean the vector comprised of the homogeneous parts of $\ch E$.

$$  \ch SE = \begin{bmatrix} \rk SE \\ \det SE \\ \chn_2 SE \end{bmatrix} =
\begin{bmatrix} -1 & \fdeg & 0 \\
2\hat f  & -1 - \hat f \circ \fdeg & \hat f \circ \deg \\
0&0&-1 \end{bmatrix}
\begin{bmatrix} \rk E \\ \det E \\ \chn_2 E \end{bmatrix} = A_S (\ch E)
\mbox{.} $$

Reducing to Bridgeland's setup, we get a simpler looking $2\times 2$ matrix:
$$  \begin{bmatrix} \rk SE \\ \fdeg SE \end{bmatrix} =
\begin{bmatrix} -1 & 1 \\ 0 & -1 \end{bmatrix}
\begin{bmatrix} \rk E \\ \fdeg E \end{bmatrix}
= B_S \begin{bmatrix} \rk E \\ \fdeg E \end{bmatrix}
\mbox{.} $$


\begin{Lem}
\label{matrix_S}
   The matrix $A_S$ is equal to:
    $$ A_S =
    \begin{bmatrix} -1 & \fdeg & 0 \\
    2\hat f  & -1 - \hat f \circ \fdeg & \hat f \circ \deg \\
    0&0&-1 \end{bmatrix}
    \mbox{.} $$
\end{Lem}
\begin{Lem}
\label{matrix_Sprime}
    The negative inverse of $A_S$ is equal to:
    $$ -A_S^{-1} = A_{S'} =
    \begin{bmatrix} 1 & \fdeg & 0 \\
    2\hat f  & 1 + \hat f \circ \fdeg & \hat f \circ \deg \\
    0&0&1 \end{bmatrix}
    \mbox{.} $$
\end{Lem}

\begin{proof}
    The author used formula with Schur complements to compute the inverse, but the reader can verify the result by direct calculation noting that $\fdeg \circ \hat f = 0$.
\end{proof}



%%%
\subsubsection{Action of $T$ on Chern classes}
%%%


For a fixed line bundle $L$ on $X$, the functor $T_L$ is a twist by $L$. Chern character is multiplicative with respect to tensor products, so we use this to calculate $\ch T_L E$. Again, let us write $\ch E = r + E_1 + E_2$: 
\begin{equation*}
\begin{split}
  \ch T_L E &= \ch E . \ch L =
    (r + E_1 + E_2).\left(1 + L + \frac{L^2}{2}\right) =\\
    &= r + (E_1 + rL) + \left(E_2 + L.E_1 + \frac{rL^2}{2}\right)
\mbox{.} \end{split}
\end{equation*}


Writing the action of $T_L$ as a matrix, we get:
$$  \ch T_L E =
\begin{bmatrix} 1 & 0   & 0 \\
\hat L & 1             & 0 \\
\frac{\hat L^2}{2}       & \hat L   & 1 \end{bmatrix}
\ch E = A_{T_L}(\ch E)
$$

The inverse of this matrix can be easily computed:
$$  A_{T_L} =
\begin{bmatrix} 1 & 0   & 0 \\
-\hat L & 1             & 0 \\
\frac{\hat L^2}{2}       & -\hat L   & 1 \end{bmatrix}
$$

In Bridgeland's setup, this reduces to:
$$  \begin{bmatrix} \rk T_L E \\ \fdeg T_L E \end{bmatrix} =
\begin{bmatrix} 1 & 0 \\
\fdeg L & 1 \end{bmatrix}
\begin{bmatrix} \rk E \\ \fdeg E \end{bmatrix} =
B_{T_L} \begin{bmatrix} \rk E \\ \fdeg E \end{bmatrix}
$$




==> body/conventions.tex <==
\chapter{Notation}
\label{notation}



%%%
%%%
\section{Derived functors and derived categories}
%%%
%%%



\begin{Conv}
    We write $(-)^\vee$ for the derived dual of a sheaf and $-\otimes -$ for the derived tensor product.
    Given a morphism of schemes $f : X \to Y$, we denote by $f_*$ and $f^*$ the derived functors of pushforward and pullback, respectively.
\end{Conv}

Note however that we distinguish between $\mathrm{Hom}$ and $\mathrm{RHom}$.

\begin{Conv}
    When, very rarely, we want to work with the classical functors instead of derived, we write $\Lab f^*$ for the nonderived pullback and $\Rab f_*$ for nonderived pushforward.
\end{Conv}



%%%
%%%
\section{Grothendieck groups and Chern characters}
%%%
%%%



For the moduli theory of sheaves, we generally need a way to fix a numerical characteristic of the sheaves in question in order to obtain any finiteness results.
So we will recall certain conventions, which we believe to make the exposition more concise and straightforward. In particular, it will enable us to summarize the known cases in a uniform way.

\begin{Not}
Here we introduce notation for variants of K-theory that we will use in the paper.
\begin{itemize}
    \item Let $\K X$ denote the Grothendieck group of perfect complexes on a noetherian stack $X$. When $X$ is a smooth projective variety, then the category of perfect complexes coincides with the bounded derived category of coherent sheaves $\Db X$.
    \item Let $\Kt X$ denote the zeroth topological K-theory of $X$.
    \item Let $\Kor X$ denote the zeroth oriented topological K-theory of $X$. Rough\-ly speaking, it lies between the algebraic K-theory $\K X$ and the topological K-theory, or more precisely, it allows to fix the determinant of a sheaf, unlike $\Kt X$.
    \item Let $\Korth X$ denote the zeroth  oriented orthogonal topological K-theory of $X$. It adds a nondegenerate symmetric bilinear form to the oriented K-theory $\Kor X$.
    \item Let $\Ksp X$ denote the zeroth symplectic K-theory of $X$. Symplectic K-theory, in addition to caring about topological classes, also fixes a choice of a symplectic form, that is a nondegenerate morphism from the second exterior power to some line bundle.
\end{itemize}
\end{Not}

\begin{Not}
Let $\Chow X$ denote the Chow ring of a smooth projective variety $X$.
\end{Not}

It is well-known that there is a function called Chern character $\ch : \Db X \to \Chow X$, from objects of the derived category to the Chow ring, that factors as a ring homomorphism through the Grothendieck group: $\ch : \K X \to \Chow X$.

We can summarize the relations between the K-groups in the following diagram:
\begin{diagram}
        &       &       &       & \Chow X   \\
        &       &       & \ruTo^{\ch}       \\
\Db X   & \rTo  & \K X  & \rTo  & \Kor X
        & \rTo  & \Kt X \\
        &       &       & \ruTo &
        & \ruTo \\
        &       & \Korth X &    & \Ksp X    \\
\end{diagram}
Note that the Euler pairing descends to each of the K-groups by taking representative complexes $E$ and $F$ and computing Euler characteristic of their derived tensor product:
$$\chi(E \otimes F) \deq \chi \left( \RGamma(E \otimes F) \right)
\mbox{.}$$

\begin{Conv}
We will call a vector $v$ in any K-theory $\Kany X$ a fixed
\emph{numerical characteristic}, or
\emph{K-theory class}. When we need to be specific, we will add adjectives algebraic, topological, oriented topological or symplectic to refer to the corresponding variants of K-theory.
\end{Conv}

Our notation will be unambigous. When, in the setting of smooth projective varieties, we want to work with Chern classes, we will write $\cn_i(v)$, and the Chern character of the numerical characteristic $v$ is denoted by $\ch v$. Note that we can pass to considering topological cycles, so we can write Chern characters as elements of more topological K-theory classes as well. When the base field is complex numbers, it will be the usual Chern characters lying in singular cohomology.

When we want to be clear which K-theory we are working with, we write $v\valg$ for algebraic, $v\vt$ for topological, and analogously $v\vor$, $v\vorth$ and $v\vsp$ for oriented, oriented orthogonal and symplectic K-theory classes, respectively.



%%%
%%% %%%
\section{Classical formulation of the Strange Duality}
%%% %%%
%%%


Let $X$ be a smooth complex projective variety.
Let us choose a polarization $H$ of $X$ and a class $v \in \K X$. Let $\Mc_v$ denote the moduli space of Gieseker $H$-semistable sheaves of class $v$. More generally, one can consider the moduli space of Brigdeland stable objects in $\Db X$, as Bayer and Macri do \cite{BM}.

The Grothendieck group $\K X$ comes with a natural pairing $\chi(v,w)$ -- the Euler characteristic of the $\RHom{X}{\,,}$ complex. For the purpose of setting up strange duality on K3 surfaces, we will use a slightly modified version $\chi(v \otimes w) = \chi(\bar v, w)$, where $\bar v$ denotes the class of the dualized complex -- this computes Euler characteristic of the global sections on tensor product.

\begin{Constr}
    If $v$ and $w$ are two orthogonal vectors in $\K X$, then there are two natural line bundles $\Theta_v$ on $\Mc_w$ and $\Theta_w$ on $\Mc_v$. Let $\Ec$ be a universal sheaf on $\Mc_w \times X$.
    If $p_1$ and $p_2$ are two projections $\Mc_w \times X \to \Mc_w$ and $\Mc_w \times X \to X$, then for some sheaf $F \in \Mc_v$, put:
    $$ \Theta_v = \det p_{1*} (\Ec \otimes p_2^* F) \mbox{.}$$
    With a symmetric assumption, we get $\Theta_w$ on $\Mc_v$.

    Define a subset of $\Mc_v \times \Mc_w$:
    $$  D = \left\{ (E,F) \mid h^0(E \otimes F) \neq 0
    \right\}\mbox{.}$$

    When $D$ is a divisor on $\Mc_v \times \Mc_w$, it defines a section $s$ of $\Theta_w \boxtimes \Theta_v \cong \Oc(D)$, unique up to a nonzero scalar. The section then induces a morphism:
    $$  \SD : \Hrm^0(\Theta_w)^\vee \to \Hrm^0(\Theta_v)
    \mbox{.} $$
\end{Constr}

This allows us to pose the main question of the classical Strange Duality:

\begin{Que}
When is the morphism $\SD$ an isomorphism?
\end{Que}


When it is, the sections of the theta line bundles are dual to each other in a canonical way (up to a scalar multiple).








==> body/history.tex <==
\chapter{Historical overview}
\label{history}


%%%
\section{First formulations of the Strange Duality conjecture}
%%%


Historically, the question of the Strange Duality arose in the community of mathematical physics and representation theory from the observation of ``a strange duality'' between representations of affine Lie algebras \cite{Frenkel}. Early geometric formulations concern the case of curves, and one of the first main results by Beauville-Narasimhan-Ramanan \cite{BNR} relates sections of theta line bundles on moduli spaces of line bundles and those of higher rank vector bundles. Their result is cited later in our text as Theorem \ref{BNR_thrm}. In their case theta line bundles on the moduli spaces of rank one bundles come from the theory of classical theta divisors.

Proposals of the Strange Duality conjecture can be found in the paper by Donagi and Tu \cite{DT}, where the authors compute the dimensions of the spaces of global sections of pairs of theta bundles, construct the conjectural duality map in full generality and provide numerical evidence for the conjecture. In addition, a later survey paper by Beauville \cite{Beau95} includes discussion of the conjecture and recent results.



%%%
\section{The Strange Duality theorem over curves}
%%%


Let $X$ be a smooth irreducible projective curve. We can write any numerical characteristic $v \in \Kany X$ as a pair $v = (r,L)$, where the first coordinate $r$ is the choice of a rank, and the second coordinate $L$ is either degree (when we talk about $\Kt X$) or a fixed isomorphism class of the determinant (when we talk about $\K X$ or $\Kor X$).

One of the first results relates moduli spaces of line bundles with higher rank vector bundles.

\begin{Thrm}[Beauville-Narasimhan-Ramanan \cite{BNR}, Theorem 3]
\label{BNR_thrm}
    Let $X$ be a smooth irreducible projective curve of genus $g \geq 2$. 
    Then the generalized theta locus is a divisor and the Strange Duality map is an isomorphism for the pair of vectors $v\vt = (1,g-1) \in \Kt X$ and $w\vor = (r,\Oc_X) \in \Kor X$, where $r \geq 1$.
\end{Thrm}

Beauville also proved Strange Duality for other structure groups of vector bundles. In this respect, the case of curves is very special because torsion-free sheaves are automatically locally free, so one can consider moduli spaces of $G$-bundles over curves without the need to compactify them. 

\begin{Thrm}[Beauville \cite{Beau06}, Main Theorem and Proposition 4.7]
    Let $X$ be a smooth irreducible projective curve of genus $g \geq 2$. 
    Then the generalized theta locus is a divisor and the Strange Duality map is an isomorphism for the following pairs of vectors:
    \begin{itemize}
        \item $v\vt = (1,g-1) \in \Kt X$ and
        $w\vorth = (r,\Oc_X) \in \Korth X$, where $r \geq 3$;
        \item $v\vsp = (2r,\Oc_X) \in \Ksp X$ and
        $w\vsp = (2s,\omega_X^{\otimes s}) \in \Ksp X$,
        where $s \geq 2$ and $\omega_X$ is the canonical bundle on $X$, in the following cases:
        \begin{itemize}
            \item $r=2$ and taking a line bundle $\kappa$ such that $\kappa \otimes \kappa \cong \omega_X$, we assume that either $\chi(\kappa)$ is odd or $h^0 (\kappa)=0$;
            \item $r \geq 3(g-1)$ and $X$ is general enough;
            \item $g=2$;
            \item $g=3$ and $X$ is non-hyperelliptic.
        \end{itemize}
    \end{itemize}
\end{Thrm}

Later, Belkale, Marian and Oprea started generalizing the Strange Duality to the case where both K-theory vectors have higher rank. This started the study of the so-called ``nonabelian theta functions'' -- sections of theta bundles over higher rank moduli spaces. 

\begin{Thrm}[Belkale \cite{Bel06}, Theorem 1.1]
For a generic curve $X$ of genus $g \geq 2$,
the theta locus is a divisor and the Strange Duality map is an isomorphism for a pair of vectors of the form
$v\vt = (k,k(g-1)) \in \Kt X$ and
$w\vor = (r,\Oc_X) \in \Kor X$.
\end{Thrm}

Shortly after that, Belkale extended his result from the generic statement by showing that the Strange Duality map is flat in moduli of curves, and hence has a locally constant rank.

\begin{Thrm}[Belkale \cite{Bel07}, Theorem 1.1 with Lemma A.1]
For any curve $X$ of genus $g \geq 2$,
the theta locus is a divisor and the Strange Duality map is an isomorphism for a pair of vectors of the form
$v\vt = (k,k(g-1)) \in \Kt X$ and
$w\vor = (r,\Oc_X) \in \Kor X$.
\end{Thrm}

Finally, Marian and Oprea also showed that the Strange Duality morphism is an isomorphism for any curve even without requiring the determinant to be trivial, thus answering the question of the $\GL$ vs $\SL$ Strange Duality on curves in full generality.

\begin{Thrm}[Marian-Oprea \cite{MO06}, Theorem 4]
For any curve $X$ of genus $g \geq 2$,
the theta locus is a divisor and the Strange Duality map is an isomorphism for any orthogonal pair of vectors
$v\vt \in \Kt X$ and
$w\vor \in \Kor X$.
\end{Thrm}





%%%
\section{Progress on the Strange Duality on surfaces}
%%%


\begin{Not}
Let $X$ be a smooth irreducible projective surface. We write a vector $v \in \Kany X$ in the form:
$$  v   = (\chn_0 v , \chn_1 v , \chn_2 v)
        = (\rk v , \cn_1 v , \chn_2 v)
\mbox{.} $$
Note that the third component of the vector is the degree two homogeneous component of the Chern character, not the second Chern class:
$$  \chn_2 v =
    \frac{(\cn_1v)^2}{2} - \cn_2 v
\mbox{.} $$
\end{Not}

Marian and Oprea extended the study of the Strange Duality to surfaces and obtained remarkable results about Hilbert schemes of points and moduli spaces over K3 surfaces. Their result about Hilbert schemes is so far the only known to us result that holds for any surface.

\begin{Thrm}[Marian-Oprea \cite{MO08}, Proposition 1]
\label{MO_Hilb}
For any surface $X$, for any line bundle $L$ on $X$ with $\chi(L) = n$ and no higher cohomology,
the theta locus is a divisor and the Strange Duality map is an isomorphism for a pair of vectors of the form
$v\vor = (1,\Oc_X,-k) \in \Kor X$ and
$w\vor = (1,L,\frac{1}{2} L^2 - l) \in \Kor X$, where $k$ and $l$ are positive integers that sum up to $k+l=n$.
\end{Thrm}

They used the Strange Duality for Hilbert schemes of points in conjunction with Bridgeland-style birational isomorphisms \cite{Br} to extend their result to higher rank moduli spaces on elliptic K3 surfaces. Further, they obtained a generic Strange Duality statement by a deformation argument in moduli.

\begin{Thrm}[Marian-Oprea \cite{MO10}, Theorems 1 and 1A]
Let $(X,H)$ be a generic polarized K3 surface of degree not two (that is $H^2 >2$) with $\Pic X = \Z H$. 
Consider orthogonal vectors $v$ and $w$ in $\Kt X$ such that
$\cn_1 v = \cn_1 w = H$ and
both $\chi (v)$ and $\chi (w)$ are not greater than zero.
Then the theta locus is a divisor and the Strange Duality map is an isomorphism in the following two cases:
\begin{itemize}
    \item $\rk v \geq 2$, $\rk w \geq 3$,
            $\chi(v,v) \geq f(\rk v)$ and $\chi (w,w) \geq f(\rk w)$ for
            $f(r) = 2(r-1)(r^2+1)$
    \item $\rk v = \rk w = 2$.
\end{itemize}
\end{Thrm}

In their later paper \cite{MO14}, Marian and Oprea strengthened their result on elliptic K3 surfaces.

\begin{Thrm}[Marian-Oprea \cite{MO14}, Theorem 1.1]
Let $(X,H)$ be an elliptic K3 surface of degree not two (that is $H^2 >2$) with fiber class $f$ and such that $H.f = 1$.
Consider orthogonal vectors $v$ and $w$ in $\Kt X$ such that
$\cn_1 v = \cn_1 w = H$ and
$\chi (v,v) + \chi (w,w) \geq 2(\rk v + \rk w)^2$.
Then the theta locus is a divisor and the Strange Duality map is an isomorphism.
\end{Thrm}


Around same time, Bayer and Macri proved that the Strange Duality morphism is either zero or an isomorphism when the bilinear pairing is defined as usual Euler form. They worked with moduli spaces of Bridgeland stable objects in a twisted derived category of a K3 surface, and assumed in addition that one of the vectors is isotropic, so the corresponding moduli space is a (possibly different) K3 surface.


We would also like to make the reader aware that there is ongoing work by numerous people on the Strange Duality over other surfaces, for example $\PS^2$, abelian and del Pezzo surfaces, as well as other surfaces. Yet we do not consider them here because these cases are out of the scope of the current work, however interesting they might be.


